Low-complexity Linear Multicast Beamforming for Cache-aided MIMO Communications

A practical and scalable multicast beamformer design in multi-input multi-output~(MIMO) coded caching~(CC) systems is introduced in this paper. The proposed approach allows multicast transmission to multiple groups with partially overlapping user sets using receiver dimensions to distinguish between different group-specific streams. Additionally, it provides flexibility in accommodating various parameter configurations of the MIMO-CC setup and overcomes practical limitations, such as the requirement to use successive interference cancellation~(SIC) at the receiver, while achieving the same degrees-of-freedom~(DoF). To evaluate the proposed scheme, we define the symmetric rate as the sum rate of the partially overlapping streams received per user, comprising a linear multistream multicast transmission vector and the linear minimum mean square error~(LMMSE) receiver. The resulting non-convex symmetric rate maximization problem is solved using alternative optimization and successive convex approximation~(SCA). Moreover, a fast iterative Lagrangian-based algorithm is developed, significantly reducing the computational overhead compared to previous designs. The effectiveness of our proposed method is demonstrated by extensive simulations.

==> Achievable_DoF.tex <==
CC techniques are shown to provide the total DoF of $t+1$ in SISO setups~\cite{maddah2014fundamental}. This total achievable DoF is increased to $t+L$ in a MISO setup with the spatial multiplexing gain of $L$ at the transmitter~\cite{shariatpanahi2018physical}, and is shown to be optimal with uncoded cache placement and single-shot data delivery~\cite{lampiris2018resolving}. Denoting the DoF as the number of parallel data streams (and not the number of users),\footnote{Note that defining the DoF as the number of streams does not contradict its conventional definition in the SISO-CC and MISO-CC literature, as in both cases every user can receive only one stream per transmission.} in~\cite{salehi2021MIMO}, it is shown that if $\frac{L}{G}$ is an integer, the total DoF of a MIMO-CC setup can reach $Gt+L$, where $G$ is the spatial multiplexing gain at the receiver side. 

%In this paper, we take a closer look at the DoF of MIMO-CC setups and provide a better bound, also supporting the case of non-integer $\frac{L}{G}$.

Consider a MIMO-CC network with coded caching gain $t$ and spatial multiplexing gains of $L$ and $G$ at the transmitter and receivers, respectively. The number of users $K$ is not smaller than $t+L$.
%a sufficiently large number of users $K \ge t+L$, where the coded caching gain is $t$, and spatial multiplexing gains at the transmitter and receivers are $L$ and $G$, respectively. Assume 
Assume in every transmission, we serve a total number of $\Omega$ users, and each user wants to decode $\beta \le G$ streams simultaneously. The goal is to maximize $\Omega \times \beta$ while assuring that decoding all the parallel streams is possible and not limited by interference.
%can be decoded with limited interference.

Consider a specific user $k$ receiving data during an arbitrary transmission interval. 
%Consider a specific user $u_k$ receiving data in a sample transmission. 
With coded caching gain $t$, the interference caused by every stream sent to user $k$ can be removed by cache contents at up to $t$ users. Moreover, as $\beta \le G$, the inter-stream interference among these streams can be suppressed by receiver-side processing. So, for successful, not interference-limited decoding,
%with limited interference, 
the interference caused by streams sent to user $k$ should be suppressed by transmitter-side precoding over every stream intended for the rest of $\Omega-t-1$ target users. As a result, we should have $L-1 \ge \beta(\Omega-t-1)$, or equivalently
\begin{equation}
    \Omega \le \big\lfloor \frac{L-1}{\beta} \big\rfloor+t+1,
\end{equation}
where the floor operation is used to ensure the upper bound is an integer. As a result
\begin{equation}\label{eq:total_DoF}
    \mathrm{DoF}_{\max} = \max_{\beta \le G} \beta \big\lfloor \frac{L-1}{\beta} \big\rfloor+ \beta(t+1).
\end{equation}
It can be shown that the function inside the $\max$ operation is \emph{not} a monotonic function of $\beta$, and hence, the maximum DoF is not necessarily achieved at $\beta = G$ (for example, consider the case $L=16$, $G=4$, $t=1$, where the DoF of~21 is achieved with $\beta = 3$, while with
$\beta = G = 4$, the DoF is~20). 
Nevertheless, setting $\beta = G$ gives us a quick metric to calculate an achievable DoF value $\mathrm{DoF}_G = G \lfloor \frac{L-1}{G} \rfloor+ G(t+1)$. %Denoting this DoF value as $\mathrm{DoF}_G$, we have
% \begin{equation}
% \label{eq:total_DoF}
%     \mathrm{DoF}_G = G \big\lfloor \frac{L-1}{G} \big\rfloor+ G(t+1).
% \end{equation}
%and the maximum achievable DoF is
%\begin{equation}
%\label{eq:total_DoF}
%    G(\big\lfloor \frac{L-1}{G}\big\rfloor + t + 1) .
%\end{equation}
%
For example, if $L=3$, $G=\beta=2$, and $t=1$, $\mathrm{DoF}_{G}=6$ is achievable. Note that with the MIMO-CC scheme in~\cite{salehi2021MIMO}, we need at least $L=4$ to achieve the same DoF. So, our scheme not only 
relaxes the integer constraint on $\frac{L}{G}$ 
%only provides an achievable DoF for non-integer $\frac{L}{G}$ values 
but also shows that the gain boost of MIMO-CC setups is possible with smaller transmitter-side spatial multiplexing gains than suggested in~\cite{salehi2021MIMO}. In Section~\ref{section:NumRes}, we confirm the achievability of the DoF value in~\eqref{eq:total_DoF} through simulations. 

%Further elaboration on DoF analysis is left for future research.

%Given an IID SISO channel and cache-enabled users with a coded caching gain $t$, one can serve $t+1$ users or include $t+1$ independent data streams within a single transmission. Hence, the achievable DoF can be increased from one to $t+1$~\cite{maddah2014fundamental}. Assuming the effect of the multi-antenna case, the cache-aided MISO setting could reveal a DoF of $t+L$~\cite{shariatpanahi2016multi}. %The achieved DoF represents the cumulative effect of the spatial multiplexing gain at the transmitter side, and the coded cache gain $t$. 
%Let's consider multistream MIMO communications in the context of coded caching. Given that $|\CK|$ users are served each with G antennas, one can enumerate different scenarios, which are elaborated on in the following.   
%\begin{itemize}  
%\item Symmetric scenario for $ L = G$ where $\eta  = \frac{L}{G} = 1$. When we encounter this case, we can decompose the MIMO system to $G$ parallel equivalent SISO system. Recalling the SISO-CC, we can serve $t+1$ 
% independent streams at each time instant. Thus the achievable DoF would be $G \times (t + 1 ) = Gt + G $.      
% \item Non-symmetric scenario for $ L > G$ where $L$ and $G$ is divisible and $\eta  = \frac{L}{G} $ is an integer value. The MIMO system reduces to a $G$ parallel equivalent MISO system when faced with such a case. For each so-called virtual MISO system, we have $L' = \eta = \frac{L}{G}$ spatial multiplexing gain at the transmitter side. Consequently, it will be possible to serve $t + L'$ or $ t + \eta $ 
% independent streams at each time instant simultaneously. The DoF attained would therefore be $G \times (t + L' ) = Gt + G \eta = Gt + L $~\cite{salehi2021MIMO}.

% \item An arbitrary pair of $L$ and $G$, where $ L > G$ and $L$ and $G$ can be either divisible or non-divisible.
 %For an arbitrary $L$ and $G$, where $ L > G$ and $L$ and $G$ could be either divisible or non-divisible;
% It has been demonstrated in the previous two cases that if $\frac{{L}}{G}$ is divisible~\cite{salehi2021MIMO}, then we could achieve a DoF of $Gt + L$.
% Furthermore, we will demonstrate that even if one picks a new number of TX antennas or considers a lower spatial multipexling gain at the transmitter side  $\bar{L}$ such that $\bar{L} < {L}$ leads to a non-divisible $\frac{\bar{L}}{G}$, still a DoF of $Gt + L$ is achievable.
% This is a valid assumption if $ \lceil\frac{\bar{L}}{G}\rceil  = \frac{{L}}{G}$ is satisfied. % still a DoF of $Gt + L$ is achievable. 
% Our discussion of this case is given in the following lemma. 
% \begin{lemma}
% If $L > (|\CK| - (t+1))G$, then the achievable DoF is $\text{DoF} \geq XG$.
%\end{lemma}

 %\begin{proof}
 %In light of the definition of DoF at asymptotically large SNRs, we consider a zero-forcing scheme on the transmitter side. To ensure that an arbitrary number of $|\CK|$ users are simultaneously served while their codewords are decoded without interference, we have to set $L > (|\CK| - (t+1))G$. Each coded message intended for groups of size $t + 1$ users in a given transmission vector should be suppressed in the direction of the interfering users, enumerated as $|\CK| - (t+1)$. In the meantime, each user is able to resolve $G$ received streams, thereby benefiting from a DoF of $G$. 
 %It is deemed necessary, therefore, that $L$ must be greater than the total interference $(|\CK| - (t+1))G$ in order to cancel signals at the non-desired users. Hence, the condition is justified. 
 %Therefore, $L$ need to be larger than total interference $(|\CK| - (t+1))G$ to allow null at the non-desired users.    
% The reduction of $t+1$ from $|\CK|$ reflects that cache-assisted interference cancellation has been applied to the served users. %receives data through a rank-$G$ channel
  %In this way, since each user can resolves $G$ received stream, therefore each can potentially achieves a DoF of $G$.
  %To this end, we can achieve a total DoF of  $|\CK|G$. To reach this achievable DoF, $|\CK|$ must satisfy the following equation: $|\CK| < \frac{L}{G} + t + 1 $. 
  %Regarding the condition for the achievable DoF, $X$ should sastisfy $|\CK| < \frac{L}{G} + t + 1 $. 
 %One can recognize that the number of served users $|\CK|$ is a determining factor, and if we exceed this value, the achievable DoF will decrease.
%\end{proof}
  
 
%\end{itemize}
%As a consequence of the last option, a delivery scheme is efficiently planned based on the selected number of users and SNR.
%Thus, the last case generally plans a delivery scheme based on the selected number of users and SNR. %In fact in the lower SNR values we might lose some DoF. 


==> Data/CCMAC.tex <==
SNR	B10OPT	B5OPT	B2OPT	B1OPT	B10toB1OPT	B2toB1OPT	B5toB1OPT
0	3.019496031	3.237992628	3.050747707	2.928696004	3 	4 	11 
5	6.006190989	6.203754341	5.843921052	5.537773058	8 	6 	12 
10	10.05986468	10.15248871	9.617257408	9.103326084	11 	6 	12 
15	15.12031657	15.05797721	14.20208891	13.39369048	13 	6 	12 
20	21.17906799	20.85934331	19.47841259	18.23805437	16 	7 	14 
25	27.93463344	27.3101688	25.33555066	23.39801623	19 	8 	17 
30	35.03084845	34.15059121	31.62450906	28.8261219	22 	10 	18 


==> Data/CCMC.tex <==
SNR	P15OPT	P12OPT	P6OPT	P3OPT	P15toP3OPT	P12toP3OPT	P6toPeOPT
0	3.019496031	2.942123949	2.24876639	2.042137213	48 	44 	10 
5	6.006190989	5.682989345	4.483561279	4.064630863	48 	40 	10 
10	10.05986468	9.36986002	7.625063013	6.907223017	46 	36 	10 
15	15.12031657	14.05027524	11.79554043	10.66633933	42 	32 	11 
20	21.17906799	19.84333005	17.17364819	15.52134839	36 	28 	11 
25	27.93463344	26.57432536	23.62563627	21.43007544	30 	24 	10 
30	35.03084845	33.78025068	30.73168825	28.10399695	25 	20 	9 


==> Data/CCMUX.tex <==
SNR	t2OPT	t1OPT	t0OPT	t2tot0OPT	t1tot0OPT	t2tot0TH	t1tot0TH
0	3.019496031	2.545210477	1.722927977	75 	48 	50 	25 
5	6.006190989	4.816306824	3.158179176	90 	53 	50 	25 
10	10.05986468	7.888027322	5.013348108	101 	57 	50 	25 
15	15.12031657	11.82856724	7.360721638	105 	61 	50 	25 
20	21.17906799	16.6813452	10.32663768	105 	62 	50 	25 
25	27.93463344	22.24682991	13.92519769	101 	60 	50 	25 
30	35.03084845	28.16252698	18.02488853	94 	56 	50 	25 


==> Data/SBF.tex <==
SNR	A4OPT	A3OPT	A2OPT	A1OPT	A4toA1OPT	A3toA1OPT	A2toA1OPT	A4toA1TH	A3toA1TH	A2toA1TH
0	3.019496031	3.255389193	3.19462742	3.03884808	-1 	7 	5 	100 	67 	33 
5	6.006190989	6.344362273	6.195238781	5.633862543	7 	13 	10 	100 	67 	33 
10	10.05986468	10.54495756	10.12109494	8.766504708	15 	20 	15 	100 	67 	33 
15	15.12031657	15.68325763	14.54256121	12.12092439	25 	29 	20 	100 	67 	33 
20	21.17906799	21.33266891	19.13520889	15.54965486	36 	37 	23 	100 	67 	33 
25	27.93463344	27.14877531	23.76366594	19.00050556	47 	43 	25 	100 	67 	33 
30	35.03084845	32.9969125	28.39100504	22.45708665	56 	47 	26 	100 	67 	33 
35

==> Data/SMUX.tex <==
SNR	L4OPT	L3OPT	L2OPT	L1OPT	L4toL1OPT	L3toL1OPT	L2toL1OPT	L4toL1TH	L3toL1TH	L2toL1TH	L4toL3OPT	L4toL3TH	L4toL2OPT	L4toL2TH
0	3.019496031	2.49186387	1.423904776	0.597396735	405 	317 	138 	100 	67 	33 	21 	20 	112 	50 
5	6.006190989	5.008934723	3.162012335	1.512479737	297 	231 	109 	100 	67 	33 	20 	20 	90 	50 
10	10.05986468	8.497909094	5.709079172	3.223654597	212 	164 	77 	100 	67 	33 	18 	20 	76 	50 
15	15.12031657	12.96424947	8.899232124	5.738082738	164 	126 	55 	100 	67 	33 	17 	20 	70 	50 
20	21.17906799	18.26457795	12.76218425	8.807504004	140 	107 	45 	100 	67 	33 	16 	20 	66 	50 
25	27.93463344	24.06475332	17.17230996	12.16160646	130 	98 	41 	100 	67 	33 	16 	20 	63 	50 
30	35.03084845	30.04428564	21.91653976	15.63077287	124 	92 	40 	100 	67 	33 	17 	20 	60 	50 
35

==> Data/STYPE.tex <==
SNR	L4A4OPT	L4A4ZF	L4A2OPT	L4A2ZF	L4A4OPTtoZF	L4A2OPTtoZF
0	3.019496031	0.442695864	3.19462742	1.76642666	582 	81 
5	6.006190989	1.342893157	6.195238781	4.218965827	347 	47 
10	10.05986468	3.768993242	10.12109494	8.022700117	167 	26 
15	15.12031657	8.9253664	14.54256121	12.54641351	69 	16 
20	21.17906799	16.63372103	19.13520889	17.25074781	27 	11 
25	27.93463344	25.62381906	23.76366594	21.94334747	9 	8 
30	35.03084845	34.2407576	28.39100504	26.6036158	2 	7 


==> Figs/data.tex <==
SNR	RsymLG32K3t1ISITcov	RsymLG32K3MMSESIC			RsymLG32K3LMMSE		RsymLG42K3t1ISITcov			RsymLG42K3MMSESIC			RsymLG42K3LMMSE			RsymLG32K3LMMSEKKT			RsymLG32K3ZF		RsymLG42K3LMMSEKKT			RsymLG64K420LMMSEKKT			RsymLG74K420LMMSEKKT			RsymLG73K420LMMSEKKT			RsymLG63K420LMMSEKKT			RsymLG42K3ZF			RsymL2G2K2t1cov		RsymLMMSEmultistreamL2G2K2t1				RsymLMMSEsinglestreamL2G2K2t1				RsymLMMSEmultistreamL8G4K3t1				RsymCovL8G4K3t1			RsymLMMSEsinglestreamL8G4K3t1				RsymproposedL8G4K4LMMSE				RsymCovL5G4K3t1			RsymproposedLMMSEL5G4K3t1				RsymproposedcovL6G4t2omg4				RsymproposedLMMSEL2G2omg2t1unicasting					RsymproposedCovL2G2omg2t1unicasting					RsymproposedLMMSEL2G2t1omg2					RsymproposedLMMSEL16G4t1omg5				RsymproposedLMMSEL6G4t0omg4			
																																																																																																	
0	5.3365	5.155871462			4.286304845		6.368072742			6.295184266			5.366			4.445386289			1.014394465		5.612811071			14.72973225			16.05390468			12.86568453			11.7813			2.0687			3.6949		3.6324					4.0999				13.1967				13.8776			13.1158				13.4936			10.8459			10.1912				18.4667					2.3698					2.8452					2.840568037					20.03229847				7.374965562		
5	10.1285	9.627746908			7.546404254		11.90574618			11.57479304			10.2109			8.07592709			2.744632086		10.50570254			27.43508453			29.78830284			23.97615411			21.5379			5.288			6.811		6.669					7.0231				23.4761				25.2802			22.1641				24.9845			19.8351			18.4914				34.3507					4.5581					5.528					5.464228094					35.96964044				13.04432827		
10	16.5253	15.52595966			12.42912228		19.35609748			18.89725902			17.1813			13.00316962			6.391043185		17.26994241			44.74465665			47.90019689			39.63979366			35.6726			11.2387			11.0363		10.8893					10.413				36.9815				40.3851			32.4828				40.6831			31.9366			29.0468				55.838					7.5184					9.2799					9.045829524					56.39875426				20.02855348		
15	24.0321	22.48949621			18.68081926		28.32135207			27.7317032			25.6506			18.57993309			12.44784526		25.82016812			64.9039887			68.47440945			58.6044018			53.2958			19.7153			16.3266		16.1615					13.999				53.7595				58.2191			43.3038				59.5164			46.4542			40.6405				81.1861					10.9255					14.1744					13.79933789					78.81724526				27.63015542		
20	32.4362	30.26114845			25.73387483		38.36197593			37.48632488			35.284			25.51354743			20.62635136		35.73827386			86.28193517			89.95075643			79.39695807			73.2548			29.7273			22.5407		22.4					17.6551				73.0311				78.225			54.252				80.2317			62.3754			52.5488				108.8675					14.5148					20.1533					19.72999638					109.9746044				35.05444451		
25	41.6948	38.59334415			33.68214794		49.01941028			47.87352765			45.6354			33.69018903			30.22308829		46.30414142			108.034779			111.710456			100.8427299			94.4109			40.4233			29.3885		29.2652					21.3349				93.7875				99.533			65.1097				101.6557			78.8102			64.3329				138.6481					18.1597					26.894					26.46651276					135.1328232				41.33117885		
30	51.7005	47.56752368			42.96937048		59.94510013			58.61208239			56.326			42.75436618			40.60689773		57.1252819			129.0867536			132.808216			122.3691413			114.3688			51.372			36.561		36.4331					25.0025				115.0608				121.4015			75.4295				122.9313			95.3402			75.5885				170.1896					21.7405					34.0278					33.59691835					158.7866404				47.37523183		


==> Figs/data_Fig3.tex <==
SNR	RsymL2G2K2t1cov		RsymLMMSEmultistreamL2G2K2t1				RsymLMMSEsinglestreamL2G2K2t1				RsymLMMSEmultistreamL8G4K3t1				RsymCovL8G4K3t1			RsymLMMSEsinglestreamL8G4K3t1				RsymproposedL8G4K4LMMSE				RsymCovL5G4K3t1			RsymproposedLMMSEL5G4K3t1				RsymproposedLMMSEsinglestreamL5G4K3t1				
																																					
0	3.6949		3.6324					4.0999				13.1967				13.8776			13.1158				13.4936			10.8459			10.1912				10.5128406				
5	6.811		6.669					7.0231				23.4761				25.2802			22.1641				24.9845			19.8351			18.4914				18.67400687				
10	11.0363		10.8893					10.413				36.9815				40.3851			32.4828				40.6831			31.9366			29.0468				28.56133074				
15	16.3266		16.1615					13.999				53.7595				58.2191			43.3038				59.5164			46.4542			40.6405				39.20547288				
20	22.5407		22.4					17.6551				73.0311				78.225			54.252				80.2317			62.3754			52.5488				50.13539057				
25	29.3885		29.2652					21.3349				93.7875				99.533			65.1097				101.6557			78.8102			64.3329				61.08710934				
30	36.561		36.4331					25.0025				115.0608				121.4015			75.4295				122.9313			95.3402			75.5885				71.51098206				


==> Figs/data_Globcom.tex <==
SNR 	RsymLG32K3t1ISITcov	 RsymLG32K3MMSESIC  RsymLG32K3MMSE
					
0	5.3365	5.1562   4.2877
5	10.1285	9.6274 	7.5527
10	16.5253	15.5328	 12.4468
15	24.0321	22.4945	 18.6496
20	32.4362	30.2347	 25.7339
25	41.6948	38.6218	 33.8356
30	51.7005	47.4762	 42.7128


==> Transmission_Strategy.tex <==
%Here we provide examples of how the transmission user target size affects the problem and what we expect in each case on the covariance matrix rank behavior.
In this section, we analyze the impact of various multigroup multicast transmission configurations and reveal how the chosen transmission strategy can influence both the MIMO-CC system design and its performance. We assume a content delivery scenario illustrated in Fig.1, where a transmitter with $L$ antennas should fulfill requests from $K = 10$ users, each equipped with $G =2$ antennas.
We compute the symmetric rate $R_{sym}$ in \eqref{eq:TX_signal}, taking into account the number of transmission vectors and codeword lengths, while assuming the same content placement strategy as in~\cite{maddah2014fundamental}.  It should be noted that, as discussed in Section~\ref{section:sys_model}, we need to further split each subfile $W_{\CP}$ into $\binom{K-t-1}{\Omega-t-1}$ smaller chunks $W_{\CP}^q$. However, as a matter of simplicity, chunk indices $q$ are ignored here since they do not have any influence on the algorithm's behavior. Moreover, throughout this analysis, we focus on the transmission vector in a single time slot, even though the data transfer takes place over multiple consecutive time slots (in each slot, $\Omega$ users are served). Below, we illustrate various configurations through a number of examples to provide a better understanding.
%Here, we examine the configuration of multigroup multicast transmissions for various setups, and illustrate how the size of the transmission target affects the problem.
%We consider multigroup multicast covariance matrix design for different setups explained in various examples.  
%\subsection{Scenario 1: $L \geq 3$, $G = 2$, and $t=1$} 
%\subsubsection{ $|\CK| = 3$ Selected User Served }

\begin{exmp}
    \label{exmp:x3serv}
\normalfont
In this example, the BS has $L=4$ antennas and serves  $\Omega = 3$ users, and the CC gain is $t = 1$ (i.e., $\textrm{DoF} =6$). For notational simplicity, let us assume that $ A$, $B$, and $C$ denote the files requested by users 1-3, respectively.
%$M=1$ () from a library $\{A, B, C\}$ of size $N = 3$. %Regardless of whether actual requests are known beforehand, we consider that in the cache content placement phase each user can cache $M=1$ ($t = 1$).
%
For this setup, the multicast transmission vector for users~1-3 can be written as
%Following the setup, the general multicast transmission signal vector is defined as 
\begin{IEEEeqnarray}{lll}\label{eq:Psig}
		{\Bx}= {\Bx}_{1,2}   + {\Bx}_{1,3} + {\Bx}_{2,3},
	\end{IEEEeqnarray}
where each signal is proportional to its transmitted message, i.e., $ {\Bx}_{1,2} \propto (A_2\oplus B_1) $, $ {\Bx}_{1,3} \propto (A_3\oplus C_1)  $, $ {\Bx}_{2,3} \propto (B_3\oplus C_2) $.\footnote{As a special case, in~\eqref{eq:Psig}, we may use linear transmit precoders $ \Bw_{\mathcal{T}}$, defined by indices~$\mathcal{T} \in \{\{1,2\}, \{1,3\}, \{2,3\}\}$, to get the transmission vector
		${\Bx}= (A_2\oplus B_1)\Bw_{1,2} + (A_3\oplus C_1)\Bw_{1,3} + (B_3\oplus C_2) \Bw_{2,3}$~\cite{tolli2018multicast}.}
% In Appendix \ref{A}, a special case of (\refeq{eq:Psig}) can be found.
 %that is a linear transmit precoding, where the transmit vector is expressed as~\cite{tolli2018multicast}:   
%  \begin{IEEEeqnarray}{lll}\label{eq:Linear Precoder}
% 		{\Bx}(1)= (A_2\oplus B_1)\Bw_{1,2} + (A_3\oplus C_1)\Bw_{1,3} + (B_3\oplus C_2) \Bw_{2,3} ,\nonumber\\
% 	\end{IEEEeqnarray}
% In (\refeq{eq:Linear Precoder}) $ \Bw_{\mathcal{T}}$ denotes multicast beamformer, $\mathcal{T} \in \{\{1,2\}, \{1,3\}, \{2,3\}\}$. 
Then, the received signals at users 1-3 can be expressed as:
\begin{IEEEeqnarray}{lll}\label{eq:rx_sig}
		\By_1 = \underline{\BH_1 {\Bx}_{1,2}}   + \underline{\BH_1{\Bx}_{1,3}} + \BH_1 {\Bx}_{2,3} + \Bz_1\; ,\nonumber\\
  \By_2 = \underline{\BH_2 {\Bx}_{1,2}} + \underline{\BH_2 {\Bx}_{2,3}} + \BH_2{\Bx}_{1,3} + \Bz_2\; ,\\
  \By_3 = \underline{\BH_3 {\Bx}_{1,3}} + \underline{\BH_3 {\Bx}_{2,3}} + \BH_3{\Bx}_{1,2} + \Bz_3\;\nonumber ,
\end{IEEEeqnarray}
where underlined terms correspond to the desired signals for each user.
Now, if we consider user~1, both ${\Bx}_{1,2}$ and ${\Bx}_{1,3}$ are desired signals while
${\Bx}_{2,3}$ appears as Gaussian interference. Thus, $\By_1$ represents a Gaussian MAC channel, and user 1 can decode both of its required messages with the equal rate of
\begin{equation}
    R_{MAC}^1  = \text{min}\Big(R_{\{1,2\}}^{}, R_{\{1,3\}}^{}, \frac{1}{2} R_{{\{\{1,2\}, \{1,3\}\}}}^{}\Big),
\end{equation}
%$$,
where $R_{{\{\{1,2\}, \{1,3\}\}}}^{} = R_{\{1,2\}}^{} + R_{\{1,3\}}^{}$, and $R_{\{1,2\}}^{}$ and $R_{\{1,3\}}^{}$ correspond to ${\Bx}_{1,2}$ and ${\Bx}_{1,3}$, respectively. Using this example as a guide, $\CK  =\{1,2,3\}$, $\mathsf S^{\CK} = \{\{1,2\}, \{1,3\}, \{2,3\}\}$, $\mathsf S_1^{\CK}  = \{\{1,2\}, \{1,3\}\}$, $\bar{\mathsf S}_1^{\CK}  = \{\{2,3\}\}$, and $\mathsf B $ could be selected as $\{\{1,2\}\}$, $ \{\{1,3\}\}$, or $  \{\{1,2\}, \{1,3\}\}$.
%Assuming that the number of transmission vectors is equal to $I=\binom{10}{3}$ and the codeword length is $\frac{1}{\binom{10}{1}\binom{8}{1}}$, total transmission time would be $ T =   \frac{{\sum_i^{120}{\frac{1}{R_i}}}}{\binom{10}{1}\binom{8}{1}}$.
% Assuming that the number of transmission vectors and the codeword length,  the symmetric rate $R_{sym}$ is computed as in \eqref{eq:TX_signal}.
% \begin{equation}
% \label{eq:symmetric_rate_ergodic_case1k31}
% R_{sym} =  \frac{10 {\binom{10}{1}\binom{8}{1}}}{{\sum_i^{120}{\frac{1}{R_i}}}}  \; ,
% \end{equation} 
Therefore, the optimum multicast transmission rate, determined w.r.t the covariance matrices, can be found by solving:
% \begin{equation}
% \label{eq:symmetric_rate_ergodic_case1k31_max}
%  R_{i}   =  \max_{\mathbf{K}_{\mathbf{x}_{\mathcal{T}}}} \min_{k\in \CK} 
%   R_{MAC}^k, \forall i \in I \;.
% \end{equation}
% The optimization problem in \eqref{eq:symmetric_rate_ergodic_case1k31_max} is relegated to Appendix \ref{B}  
%The symmetric rate maximization for $\CK = \{1,2,3\}$ with $\Omega = 3$ is expressed as 
\begin{equation}
\label{eq:P_optimum1_K3}
\begin{aligned}
&\max_{\mathbf{K}_{{\mathbf{x}}_{\mathcal{T}}}, R}  
  R \\
    &s.t.\quad R \leq \log|\mathbf{I}+\mathbf{H}_1 \mathbf{K}_{{\Bx}_{1,2}}\mathbf{H}_1^H\BQ_{1}^{-1}|, \; \\
    &\quad\:\quad R  \leq \log|\mathbf{I}+\mathbf{H}_1 \mathbf{K}_{{\Bx}_{1,3}}\mathbf{H}_1^H\BQ_{1}^{-1}|, \; \\
    & \quad\:\quad  R \leq \frac{1}{2}\log|\mathbf{I}+\mathbf{H}_1 (\mathbf{K}_{{\Bx}_{1,2} } + \mathbf{K}_{{\Bx}_{1,3} })\mathbf{H}_1^H\BQ_{1}^{-1}|,\: \\
    &\quad\:\quad R  \leq \log|\mathbf{I}+\mathbf{H}_2 \mathbf{K}_{{\Bx}_{1,2}}\mathbf{H}_2^H\BQ_{2}^{-1}|, \; \\
    & \quad\:\quad R  \leq \log|\mathbf{I}+\mathbf{H}_2 \mathbf{K}_{{\Bx}_{1,3}}\mathbf{H}_2^H\BQ_{2}^{-1}|, \; \\
    & \quad\:\quad R  \leq \frac{1}{2}\log|\mathbf{I}+\mathbf{H}_2 (\mathbf{K}_{{\Bx}_{1,2} } + \mathbf{K}_{{\Bx}_{2,3} })\mathbf{H}_2^H\BQ_{2}^{-1}|,\: \\
    &\quad\:\quad R \leq \log|\mathbf{I}+\mathbf{H}_3 \mathbf{K}_{{\Bx}_{1,3}}\mathbf{H}_3^H\BQ_{3}^{-1}|, \; \\
    & \quad\:\quad R \leq \log|\mathbf{I}+\mathbf{H}_3 \mathbf{K}_{{\Bx}_{2,3}}\mathbf{H}_3^H\BQ_{3}^{-1}|, \; \\
    & \quad\:\quad R  \leq \frac{1}{2}\log|\mathbf{I}+\mathbf{H}_3 (\mathbf{K}_{{\Bx}_{1,3} } + \mathbf{K}_{{\Bx}_{2,3} })\mathbf{H}_3^H\BQ_{3}^{-1}|, \; \\
    & \quad\:\quad \sum_{\mathcal{T} \in \{\{1,2\}, \{1,3\}, \{2,3\}\} }\text{Tr}(\mathbf{K}_{{\Bx}_{\mathcal{T}}})
	  \leq P_T ,
\end{aligned}
\end{equation}
where $\BQ_{1}  =  N_0\mathbf{I}+\mathbf{H}_1 \mathbf{K}_{{\Bx}_{2,3}}\mathbf{H}_1^H $, $\BQ_{2}  =   N_0 \mathbf{I}+\mathbf{H}_2 \mathbf{K}_{{\Bx}_{1,3}}\mathbf{H}_2^H $, and $\BQ_{3}  =   N_0\mathbf{I}+\mathbf{H}_3 \mathbf{K}_{{\Bx}_{1,2}}\mathbf{H}_3^H $.  Problem (\refeq{eq:P_optimum1_K3}) is nonconvex; however, it can be readily solved by the proposed SCA in \textbf{Algorithm 1}.
 \end{exmp}

\begin{exmp}
    \label{exmp:x4serv}
\normalfont
In this scenario, we increase the number of served users to $\Omega=4$, while keeping the transmitter-side antenna count as $L=4$ and the %each with 
CC gain as $t = 1$ (it can be seen that $\textrm{DoF} = 4$).
%requesting files from a library $\CW = \{A, B, C, D\}$ of size $N = 4$ files. 
Let us assume users 1-4 request files $A$, $B$, $C$, and $D$. Then, the general multicast transmission vector is
\begin{IEEEeqnarray}{lll}\label{eq:Psig4}
		{\Bx}= {\Bx}_{1,2}   + {\Bx}_{1,3} + {\Bx}_{1,4} +{\Bx}_{2,3} + {\Bx}_{2,4} +{\Bx}_{3,4},
	\end{IEEEeqnarray}      
where $ {\Bx}_{1,2} \propto (A_2\oplus B_1) $, $ {\Bx}_{1,3} \propto (A_3\oplus C_1) $, $ {\Bx}_{1,4} \propto (A_4\oplus D_1) $, $ {\Bx}_{2,3} \propto (B_3\oplus C_2)  $, $ {\Bx}_{2,4} \propto (B_4\oplus D_2) $, and $ {\Bx}_{3,4} \propto (C_4\oplus D_3) $. The received signal at user $k$ is expressed as 
\begin{IEEEeqnarray}{lll}\label{eq:rx_sig4}
		\By_k = \BH_k {\Bx}_{1,2}   + \BH_k{\Bx}_{1,3} + \BH_k{\Bx}_{1,4} +\BH_k{\Bx}_{2,3} +\BH_k{\Bx}_{2,4} ,\nonumber\\ \qquad\qquad+\BH_k{\Bx}_{3,4} + \Bz_k\;. 
\end{IEEEeqnarray}
In this case, each user faces a $3$-dimensional MAC channel that is characterized by three desired signals, three Gaussian interference terms, and one noise term. Calculating the optimum multicast rate and symmetric rate follows the same procedure as in the previous example. However, instead of the 9 rate constraints in~\eqref{eq:P_optimum1_K3}, the optimization problem will have 28 constraints due to the increased $\Omega$ and MAC size.
% In addition, we refer the reader to Appendix \ref{D} for additional examples. %Therefore, user $k$ can decode each of its desired signals with the rate $R_{MAC}^k =  \text{min}(R_{1}^{k}, R_{2}^{k} , R_{3}^{k}, \frac{1}{2} R_{4}^{k}, \frac{1}{2} R_{5}^{k}, \frac{1}{2} R_{6}^{k}, \frac{1}{3} R_{7}^{k})$ where the rate bounds $R_{1}^{k}$, $R_{2}^{k}$, and $R_{3}^{k}$ correspond to $\tilde{\Bx}_{k,j}$, $\forall k\neq j$, and $\tilde{\Bx}_{1,3}$, respectively. Also, given ${\CS_2} = \{4, 5, 6 \}$, and ${\CS_3} = \{7\}$ the rate bounds $R_{4}^{k}, R_{5}^{k}, R_{6}^{k}$ limit the sum rate of any combination of two transmitted multicast signals, and $R_{7}^{k}$ is the sum rate bound for 3 messages. 
 % The time needed to recover the entire file is 
 % $ T =  \frac{{\sum_i^{210}{\frac{1}{R_i}}}}{\binom{10}{1}\binom{8}{2}}$, and consequently the symmetric rate $R_{sym} = \frac{10 {\binom{10}{1}\binom{8}{2}}}{{\sum_i^{210}{\frac{1}{R_i}}}}$, where $ R_{i}$ is computed similar to \eqref{eq:symmetric_rate_ergodic_case1k31_max}. %where $ R_{i}   =  \max_{\mathbf{K}_{\mathbf{x}_{\mathcal{T}}}} \min_{k\in \CK} 
%   R_{MAC}^k$. The symmetric rate can then be computed as  
% \begin{equation}
% \label{eq:symmetric_rate_ergodic_case1k41}
% R_{sym} =  \frac{10 {\binom{10}{1}\binom{8}{2}}}{\binom{10}{4}}R_{erg}  \; ,
% \end{equation}
%  The SCA in \textbf{Algorithm 1} is employed to solve (\refeq{eq:symmetric_rate_ergodic_case1k41}).
 \end{exmp}
%\subsubsection{ $|\CK| = 5$  Selected User Served }

\begin{exmp}\label{exmp:x5serv}
    \normalfont This example addresses the special case of $L=G$ and $\Omega = {t + 1}$ in Remark~\ref{remark1}.
    %, where the multicast signal vector ${\Bx}= {\Bx}_{1,2,3}$, 
    Assume $ \Omega  = 3$, and $t = 2 $ (for this configuration, $\textrm{DoF}=3 \times G$ for any $G$). Upon transmitting signal vector $\Bx = \Bx_{1,2,3}$, the received signal vectors are 
\begin{IEEEeqnarray}{lll}\label{eq:rx_sigsymm}
  \By_1 = \BH_1 {\Bx}_{1, 2, 3} + \Bz_1\; ,\nonumber\\
  \By_2 = \BH_2  {\Bx}_{1, 2, 3} + \Bz_2\; ,\\
  \By_3 = \BH_3  {\Bx}_{1, 2, 3} +  \Bz_3\;\nonumber .
\end{IEEEeqnarray}
In this case, there is no interference and the optimal multicast rate solution is obtained by
\begin{equation}
\label{eq:P_optimum1_K1_symexm}
\begin{aligned}
&\max_{\mathbf{K}_{{\Bx}_{1, 2, 3}}, R_{}^k} \min_{k\in \CK} 
  (R_{}^1, R_{}^2, R_{}^3) \\
    &s.t.\quad R_{}^{1} \leq \log|\mathbf{I}+\mathbf{H}_1 \mathbf{K}_{{\Bx}_{1, 2, 3}}\mathbf{H}_1^H|, \; \\
    &\quad\:\quad R_{}^{2} \leq \log|\mathbf{I}+\mathbf{H}_2 \mathbf{K}_{{\Bx}_{1, 2, 3}}\mathbf{H}_2^H|, \; \\
    &\quad\:\quad R_{}^{3} \leq \log|\mathbf{I}+\mathbf{H}_3 \mathbf{K}_{{\Bx}_{1, 2, 3}}\mathbf{H}_3^H|, \; \\
    & \quad\:\quad \text{Tr}(\mathbf{K}_{{\Bx}_{1, 2, 3}})
	  \leq P_T .
\end{aligned}
\end{equation}
where the convex problem~\eqref{eq:P_optimum1_K1_symexm} could be efficiently tackled with CVX solvers. 
%Following the same procedures as in the previous examples, we have $R_{sym} = \frac{10 {\binom{10}{2}}}{{\sum_i^{120}{\frac{1}{R_i}}}}$ 
\end{exmp}

\begin{exmp}
    \label{exmp:x6serv}
\normalfont
Let us assume $L=G=2$. For different combinations of $\Omega \in \{2, 3, 4\}$ and $t \in \{1,2\}$, the possible transmission vectors are:
%In this example, assuming $L=2$ and $G=2$, we can choose the number of served users to be $\Omega = \{2, 3, 4\}$, making requests for files from $\{A-B, A-C, A-D\}$, respectively, and the CC gain $t$ is either 1 or 2. % $t \in \{1, 2\}$. 
%In this scenario, the number of served users belong to set $\Omega = \{2, 3, 4\}$, each with CC gain $t \in \{1, 2\}$, each making requests for files from $\{A-B, A-C, A-D\}$, respectively. 
%As a part of the content delivery process, users demand their required files. Then, the multicast transmission signal vectors for these setups are defined as: 
 \begin{IEEEeqnarray}{lll}\label{eq:tx_sig_xx}
\!\!\!\!\!\!\!\!\!\!\!\!{\Bx}= \begin{cases}
      {\Bx}_{1,2}, &  \Omega  = 2 , t = 1 ,\\
     {\Bx}_{1,2}   + {\Bx}_{1,3}  +{\Bx}_{2,3},& \Omega  = 3 , t = 1 ,\\
     {\Bx}_{1,2,3},                 &\Omega  = 3 ,t = 2 , \\
     {\Bx}_{1,2,3}   + {\Bx}_{1, 2, 4}  +{\Bx}_{1,3, 4} +{\Bx}_{2, 3, 4} , &  \Omega  = 4 ,t = 2,
\end{cases} 
\end{IEEEeqnarray}
which result in $\textrm{DoF}$ values of 4, 3, 6, and 4, respectively.
Note the transmission vectors for the cases $t=1,\Omega=4$ and $t=2,\Omega=2$ cannot be generated, as the condition $t+1 \le \Omega \le t+L$ must hold. %For any selection of transmission vectors in~\eqref{eq:tx_sig_xx}, the received signal at user~$k$ is always given as
%and the received signal at the individual user $k$ is given by:  
% \begin{IEEEeqnarray}{lll}\label{eq:rx_sigsym}
% 		\By_k = \BH_k {\Bx} +\Bz_k .\; 
% \end{IEEEeqnarray}
Given the multicast vectors in~\eqref{eq:tx_sig_xx}, the second and fourth signal vectors correspond to a 2- and 3-dimensional MAC channel, respectively. The symmetric rate is then calculated using the same method as in Examples~\ref{exmp:x3serv} and~\ref{exmp:x4serv}, with the only difference being that $t = 2$. The first and third signal vectors do not have an equivalent MAC channel as all users can be served with a single multicast message as elaborated in Example~\ref{exmp:x5serv}. 
%We must work through all different parameter combinations to find the optimal strategy.
\end{exmp}

\begin{exmp}
    \label{exmp:x7serv}
\normalfont
Consider a similar setup to example~\ref{exmp:x3serv} albeit with $L = 3$, which results in a non-divisible $\frac{L}{G}$. 
For different possible selections of the number of served users $\Omega = \{2, 3, 4\}$, we have the following signal vectors
 \[
{\Bx}= \begin{cases}
     {\Bx}_{1,2}   + {\Bx}_{1,3} + {\Bx}_{1,4} +{\Bx}_{2,3} + {\Bx}_{2,4} +{\Bx}_{3,4},&  \Omega  = 4 ,\\
     {\Bx}_{1,2}   + {\Bx}_{1,3}  +{\Bx}_{2,3}, &  \Omega  = 3,\\
     {\Bx}_{1,2}, &  \Omega  = 2,
\end{cases}
\]
that correspond to $\textrm{DoF}$ values of 4, 6, and 4, respectively.
Following the previous examples of multicast transmission signals, one can compute the symmetric rate similarly.
\end{exmp}


% \begin{exmp}
%     \label{exmp:x5serv}
% \normalfont Here, the number of served users increased to $\Omega = 5$, with CC gain $t = 1$.%, requesting files from $A$, $B$, $C$, $D$, $E$. 
% Similarly, users 1-5 request files $A$, $B$, $C$, $D$, $E$ during the content delivery phase. Then, the general multicast transmission signal vector is
%  	\begin{IEEEeqnarray}{lll}\label{eq:Psig5}
% 		{\Bx}= \tilde{\Bx}_{1,2}   + \tilde{\Bx}_{1,3} + \tilde{\Bx}_{1,4} + \tilde{\Bx}_{1,5} +\tilde{\Bx}_{2,3} +\tilde{\Bx}_{2,4}  +\tilde{\Bx}_{2,5} +\tilde{\Bx}_{3,4} \nonumber\\+\tilde{\Bx}_{3,5} +\tilde{\Bx}_{4,5},
% 	\end{IEEEeqnarray}      
% Accordingly, the received signal at user $k$ is  
% \begin{IEEEeqnarray}{lll}\label{eq:rx_sig5}
% 		\By_k = \BH_k \tilde{\Bx}_{1,2}   + \BH_k\tilde{\Bx}_{1,3} + \BH_k\tilde{\Bx}_{1,4} + \BH_k\tilde{\Bx}_{1,5} +\BH_k\tilde{\Bx}_{2,3} ,\nonumber\\ \qquad\qquad+\BH_k\tilde{\Bx}_{2,4} +\BH_k\tilde{\Bx}_{2,5} +\BH_k\tilde{\Bx}_{3,4} +\BH_k\tilde{\Bx}_{3,5} +\BH_k\tilde{\Bx}_{4,5}  \nonumber\\\qquad\qquad+\Bz_k,\; 
% \end{IEEEeqnarray}
% Following the same procedures as in the previous examples, we have a $4$-dimensional MAC channel and $R_{sym} = \frac{10 {\binom{10}{1}\binom{8}{3}}}{{\sum_i^{252}{\frac{1}{R_i}}}}$
% % \begin{equation}
% % \label{eq:symmetric_rate_ergodic_case1k51}
% % R_{sym} =  \frac{10 {\binom{10}{1}\binom{8}{3}}}{\binom{10}{5}}R_{erg}  \; ,
% % \end{equation}
% \end{exmp}


% %\subsection{Scenario 1: $L = 2$, $G = 2$ and $t=1$, $t = 2$} 
% \begin{exmp}
%     \label{exmp:x6serv}
% \normalfont

% In this example, the number of served users can be $\Omega = \{2, 3, 4\}$, making requests for files from $\{A-B, A-C, A-D\}$, respectively, and the CC gain is either 1 or 2. % $t \in \{1, 2\}$. 
%  %In this scenario, the number of served users belong to set $\Omega = \{2, 3, 4\}$, each with CC gain $t \in \{1, 2\}$, each making requests for files from $\{A-B, A-C, A-D\}$, respectively. 
%  As part of the content delivery process, users demand their required files. Then, the multicast transmission signal vectors for these setups are defined as: 
%  \[
% {\Bx}= \begin{cases}
%      \tilde{\Bx}_{1,2}   + \tilde{\Bx}_{1,3}  +\tilde{\Bx}_{2,3},& \text{if } \{\Omega  = 3 , t = 1 \},\\
%      \tilde{\Bx}_{1,2,3}   + \tilde{\Bx}_{1, 2, 4}  +\tilde{\Bx}_{1,3, 4} +\tilde{\Bx}_{2, 3, 4} , & \text{if } \{\Omega  = 4 ,t = 2 \}\\
%       \tilde{\Bx}_{1,2}, & \text{if } \{\Omega  = 2 , t = 1 \},\\
%       \tilde{\Bx}_{1,2,3},               & \text{if }  \{\Omega  = 3 ,t = 2 \},
% \end{cases}
% \]
% given the received signal at user $k$ is  
% \begin{IEEEeqnarray}{lll}\label{eq:rx_sigsym}
% 		\By_k = \BH_k {\Bx} +\Bz_k,\; 
% \end{IEEEeqnarray}
%  The first and second signal vectors coincide with a 2- and 3-dimensional MAC channel, respectively, and the symmetric rate is calculated in the same manner as in examples \ref{exmp:x3serv}, and \ref{exmp:x4serv} (except considering $t = 2$). The third and fourth cases, however, do not involve an equivalent MAC channel and are treated differently, as explained in Appendix \ref{C}. In fact, we need to work through all of these different parameter combinations to determine which setup achieves the maximum achievable DoF.  %Given the fourth multicast signal vector, the received signal vector is ${\Bx}= \tilde{\Bx}_{1,2,3},& \text{if }  \{|\CK|  = 3,t = 2 \}$
% % \begin{IEEEeqnarray}{lll}\label{eq:rx_sigsymm}
% %   \By(1) = \BH_1 \tilde{\Bx}_{1, 2, 3} + \Bz(1)\; ,\nonumber\\
% %   \By(2) = \BH_2 \tilde{\Bx}_{1, 2, 3} + \Bz(2)\; ,\nonumber\\
% %   \By(3) = \BH_3 \tilde{\Bx}_{1, 2, 3} +  \Bz(3)\;\nonumber ,
% % \end{IEEEeqnarray}
% % in which there is no interference and optimal solution $R_{erg}$ is obtained by
% % \begin{equation}
% % \label{eq:P_optimum1_K1_symexm}
% % \begin{aligned}
% % &\max_{\mathbf{K}_{\tilde{\Bx}_{1, 2, 3}}, R_{}^k} \min_{k\in \CK} 
% %   (R_{}^1, R_{}^2, R_{}^3) \\
% %     &s.t.\quad R_{}^{1} \leq \log|\mathbf{I}+\mathbf{H}_1 \mathbf{K}_{\tilde{\Bx}_{1, 2, 3}}\mathbf{H}_1^H|, \; \\
% %     &\quad\:\quad R_{}^{2} \leq \log|\mathbf{I}+\mathbf{H}_2 \mathbf{K}_{\tilde{\Bx}_{1, 2, 3}}\mathbf{H}_2^H|, \; \\
% %     &\quad\:\quad R_{}^{3} \leq \log|\mathbf{I}+\mathbf{H}_3 \mathbf{K}_{\tilde{\Bx}_{1, 2, 3}}\mathbf{H}_3^H|, \; \\
% %     & \quad\:\quad \text{Tr}(\mathbf{K}_{\tilde{\Bx}_{1, 2, 3}})
% % 	  \leq P_T
% % \end{aligned}
% % \end{equation}
% % where \eqref{eq:P_optimum1_K1_symexm} could be efficiently tackled with CVX solvers. 

% % Following the same procedures as in the previous examples, we have a $4$-dimensional MAC channel and 
% % \begin{equation}
% % \label{eq:symmetric_rate_ergodic_case1k51}
% % R_{sym} =  \frac{10 {\binom{10}{2}}}{\binom{10}{5}}R_{erg}  \; ,
% % \end{equation}
% \end{exmp}
% \begin{exmp}
%     \label{exmp:x7serv}
% \normalfont
%  We assume a similar setup to example~\ref{exmp:x3serv}; however, $L = 3$, which results in a non-divisible $\frac{L}{G}$. 
% Assuming that the number of served users is $\Omega = \{2, 3, 4\}$, we have the following signal vectors
%  \[
% {\Bx}= \begin{cases}
%      \tilde{\Bx}_{1,2}   + \tilde{\Bx}_{1,3} + \tilde{\Bx}_{1,4} +\tilde{\Bx}_{2,3} +\tilde{\Bx}_{2,4} +\tilde{\Bx}_{3,4},& \text{if } \{\Omega  = 4 \},\\
%      \tilde{\Bx}_{1,2}   + \tilde{\Bx}_{1,3}  +\tilde{\Bx}_{2,3}, & \text{if } \{\Omega  = 3\},\\
%      \tilde{\Bx}_{1,2}, & \text{if } \{\Omega  = 2 \}.
% \end{cases}
% \]
% %The multicast transmission signals indicate that the symmetric rate is also computed in the same manner as the previous examples. 
% In accordance with the previous examples of multicast transmission signals, the symmetric rate is also computed the same way.
% \end{exmp}
% %\subsection{Scenario 1: $L = 4$, $G = 2$, and $t=2$} 
% % \begin{exmp}
% %     \label{exmp:x8serv}
% % \normalfont
 
% %  Another example of $\eta > 1$ can be found here, in which $t = 2$  and the number of users served is set to $\Omega = \{4, 5\}$.
% %   As a consequence, we have
% %  \[
% % {\Bx}=\begin{cases}
% %      \tilde{\Bx}_{1,2,3}   + \tilde{\Bx}_{1, 2, 4} +  \tilde{\Bx}_{1, 2, 5} +\tilde{\Bx}_{1,3, 4} +\tilde{\Bx}_{1,3, 5}  \\  + \tilde{\Bx}_{1,4, 5} + \tilde{\Bx}_{2, 3, 4} + \tilde{\Bx}_{2, 3, 5} + \tilde{\Bx}_{2, 4, 5} + \tilde{\Bx}_{3, 4, 5},& \text{if } \{\Omega  = 5 \},\\
% %       \tilde{\Bx}_{1,2,3}   + \tilde{\Bx}_{1, 2, 4}  +\tilde{\Bx}_{1,3, 4} +\tilde{\Bx}_{2, 3, 4}, & \text{if } \{\Omega  = 4 \}
% % \end{cases}
% % \]
% % \end{exmp}


==> wrapup.tex <==
For MISO-native parameters:
\begin{itemize}
    \item Having larger antenna arrays is always good as it adds a whole new resource to the system.
    \item For a fixed antenna array size, at the finite-SNR regime it is better to trade the spatial multiplexing gain with the beamformer directivity. Fortunately, this does not impose any structural changes to the underlying caching scheme, i.e., we do not need to design a new CC scheme. Moreover, it only affects the second-layer subpacketization (before the transmission), and hence, this parameter can be selected instantly and over the air. \textbf{This property should be kept in mind as we design new CC schemes.}
    \item As expected, optimized beamformers always outperform zero-forcing. However, the gap between the two strategies narrows down heavily at high-SNR. The gap can also be reduced at the finite-SNR regime by reducing the spatial MUX gain. So, reducing the spatial multiplexing gain at the finite-SNR regime has also another benefit: we can use less-complex ZF beamformers if complexity is a big issue.
    \item Designing less-complex optimized beamformer designs well-tailored for CC schemes is of much interest. One interesting work is done by Nariman in~\cite{mahmoodi2021low}. However, it only applies when the CC MAC size is one.
\end{itemize}

For CC-native parameters:
\begin{itemize}
    \item Similar to the antenna count, having more memory is always good as it adds a whole new resource to the system. There is one important difference, though: the gain from having more memory is less-dependent on the SNR and can be achieved regardless of the SNR value (which makes sense, as memory-aided interference cancellation has nothing to do with the SNR value).
    \item The CC multiplexing gain also plays an important role (up to 50\%) in the achievable performance. However, this is a tricky parameter to play with: on the one hand, we have pure signal-level CC schemes that provide lots of benefits such as handling dynamicity, reduced subpacketization, easy extension to MIMO setups, etc. and on the other hand are pure bit-level schemes that provide the highest multicasting gain and hence the highest possible performance. It is a big question whether this trade-off could be tuned more gently; i.e. whether we could have some benefits of the signal-level schemes while keeping at least part of the multicasting gain. For example, the easy beamformer design is shown to be doable for some bit-level schemes (Nariman), and reduced subpacketization is also shown to be possible somehow (Soheil and Itsik). A more thorough study is highly encouraged.
    \item Increasing the MAC size provides a very small benefit but adds much to the complexity. Specifically, it requires much more complex receivers. If removing the MAC makes bit-level schemes more flexible, e.g., by allowing simpler beamformer designs for them, we should aim for that.
\end{itemize}
